Dark Matter Realism: How Referential Semantics Restricts Realism in Contemporary Fundamental Physics

Philosophers increasingly treat semantics as decisive for realism about dark matter. In this paper, I consider a recent proposal from Vaynberg (2024) anchored in the causal-descriptive theory of reference from Psillos (1999, 2012). I argue that the application of Psillos' general scientific realist framework in the local context of dark matter is misguided, partly because of the overlooked metaphysical commitments underpinning causal-descriptivism, and partly because the extension of 'dark matter' on this account includes entities we do not currently consider to be dark matter, and exclude entities that we currently consider could be dark matter. Furthermore, I argue that this discord between scientific realism and dark matter should be regarded endemic in contexts where empirical evidence is scarce: the semantic details required by the proposed scientific realism is dependent on canonical empirical confirmation, because it is against that background that scientific realism has been formulated and developed.

==> dm-realism-header.tex <==
\usepackage[automark,headsepline]{scrlayer-scrpage}
\clearpairofpagestyles
\automark{section}
\newcommand{\shorttitle}{Dark Matter Realism}
\makeatletter
\@ifundefined{shorttitle}{\newcommand{\shorttitle}{\@title}}{}
\makeatother
\renewcommand*\MakeMarkcase[1]{#1}
\ihead{\shorttitle}
\ohead{\headmark}
\setheadsepline{0.2pt}
\setkomafont{pageheadfoot}{\small\normalfont}
\cfoot{\pagemark}
\pagestyle{scrheadings}
\date{\normalsize\today}
\usepackage{microtype}
\PassOptionsToPackage{bold-style=ISO}{unicode-math}
\usepackage[T1]{fontenc}
\usepackage{libertinus}
\setkomafont{disposition}{\rmfamily\normalfont}
\setkomafont{section}{\rmfamily\large}
\setkomafont{subsection}{\rmfamily\normalsize}
\setkomafont{subsubsection}{\rmfamily\normalsize}
\setkomafont{title}{\rmfamily\LARGE}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{turnstile}
\usepackage{accents}
\usepackage{upgreek}
\usepackage{logix}
\PassOptionsToPackage{dvipsnames,svgnames,x11names,table}{xcolor}
\usepackage{xcolor}
\definecolor{footrule}{HTML}{333333}
\definecolor{linkcol}{HTML}{7D3807} 
\definecolor{rulecolor}{HTML}{333333}
\definecolor{stripeOdd}{HTML}{FFFFFF}
\definecolor{stripeEven}{HTML}{EDEDED}
\setlength{\skip\footins}{15pt plus 2pt minus 1pt}
\renewcommand\footnoterule{\kern0pt{\color{footrule}\hrule width .4\columnwidth}\kern 6.0pt}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage{tabularx}
\usepackage{array}
\usepackage{multirow}
\usepackage{transparent}
\usepackage{changepage}
\usepackage{float}
\usepackage[font=footnotesize,labelfont=bf,width=0.9\textwidth]{caption}
\captionsetup{format=plain, indention=0pt, width=0.9\textwidth}
\usepackage{indentfirst}
\setlength{\parindent}{1.5em}
\setlength{\parskip}{0pt}
\usepackage[noblocks]{authblk}
\renewcommand\Affilfont{\small}
\renewcommand\Authfont{\normalsize}
\usepackage{wrapfig}
\usepackage{tikz}
\usepackage{graphicx}
\usepackage{adjustbox}
\let\oldquote\quote
\let\endoldquote\endquote
\renewenvironment{quote}{\begin{oldquote}\small}{\end{oldquote}}
\usepackage{makecell}
\renewcommand{\cellgape}{\Gape[4pt]}
\usepackage{ragged2e}
\usepackage{stmaryrd}
\newcommand{\kcrel}{\mathrel{\lower1.05ex\hbox{$\rfloor$}\mkern-5.08mu\raise1.045ex\hbox{\reflectbox{$\rceil$}}}}
\newcommand{\PHI}{ϕ }
\numberwithin{equation}{section}
\makeatletter

\newcommand*\empraise{.25ex}
\newcommand*\empkern{-.40em}

\newcommand{\emp}{\mathrel{\mathpalette\emp@inner\relax}}
\newcommand{\emp@inner}[2]{%
  \ooalign{%
    $#1\Sigma$\cr
    \hfil\kern-\empkern \raise\empraise\hbox{$#1\circ$}\hfil\cr
  }%
}
\makeatother

==> title.tex <==
$if(title)$
\title{$title$}
$endif$

$if(subtitle)$
\subtitle{$subtitle$}
$endif$

% One \author per person
$for(by-author)$
  \author$if(it.metadata.affil-id)$[$it.metadata.affil-id$]$endif${$it.name.literal$}
$endfor$

% Affiliation list with numeric IDs
$if(by-affiliation)$
  $for(by-affiliation)$
    \affil[$it.id$]{$it.name$}
  $endfor$
$endif$

